Accelerating End-Cloud Collaborative Inference via Near Bubble-free Pipeline Optimization

End-cloud collaboration offers a promising strategy to enhance the Quality of Service (QoS) in DNN inference by offloading portions of the inference workload from end devices to cloud servers. Despite the potential, the complex model architectures and dynamic network conditions will introduce numerous bubbles (\ie, idle waiting time) in pipeline execution, resulting in inefficient resource utilization and degraded QoS. To address these challenges, we introduce a novel framework named COACH, designed for near bubble-free pipeline collaborative inference, thereby achieving low inference latency and high system throughput. Initially, COACH employs an \textit{offline} component that utilizes an efficient recursive divide-and-conquer algorithm to optimize both model partitioning and transmission quantization, aiming to minimize the occurrence of pipeline bubbles. Subsequently, the \textit{online} component in COACH employs an adaptive quantization adjustment and a context-aware caching strategy to further stabilize pipeline execution. Specifically, COACH analyzes the correlation between intermediate data and label semantic centers in the cache, along with its influence on the quantization adjustment, thereby effectively accommodating network fluctuations. Our experiments demonstrate the efficacy of COACH in reducing inference latency and enhancing system throughput. Notably, while maintaining comparable accuracy, COACH achieves up to 1.7x faster inference and 2.1x higher system throughput than baselines.

==> chap3/1/alg1.tex <==
\subsection{Offline Model Partitioning with Quantization Component}
\label{subs:alg1}

\begin{algorithm}[t]
\caption{Offline and Online Optimizations in COACH}
\label{alg:alg1}
% \KwIn{Model $G$, Calibration dataset $D$, System Profiles $P$.}
\textbf{Offline Optimization:}\\
Evaluate layer computing and transmission costs in model $G$ using calibration dataset $D$ and system profiles $P$.\\ \label{line1}
Cluster parallel layers into virtual blocks within $G$.\\\label{line2}
Determine chain flow $B_g = \{b_1, b_2, \ldots, b_n\}$ in $G$. \\
Initialize search space $F=\{B_g\}$, partitioning with quantization strategy $V^*=\emptyset$.\\ \label{line3}
\For {each chain flow $B$ in $F$}{ \label{line4}
    \For {each block $b$ in $B$}{ 
        Determine quantization precision for $b$.\\
        Calculate cost functions $f(V_B)$ and $g(V_B)$.\\
        Assess the performance of pipeline execution.\\ \label{line5}
        Update optimal strategy $V_B$ for chain flow $B$.\\ \label{line6}
        \If {$b$ is a virtual block}{ 
            Add all chain flows from $b$ to $F$.\\
        }
    }
    Update $V^*$ with $V_B$.\\  \label{line7}
}
Deploy the determined strategy $V^*$ to device and server.\\ 

\textbf{Online Acceleration:}\\
Initialize  appropriate cache $AC$ with $D$.\\ \label{line8}
Evaluate cache threshold $S_{ext}$, quantization step $\Delta Q$.\\ \label{line9}
\While {Receive task feature $T^f$}{ \label{line10}
    Compute similarity degrees $\mathbf{T}$ and task separability $S$.\\ \label{line11}
    \If{$S>S_{ext}$}{ 
        Update $T^{c\prime}_j \in AC$ according to Eq. \eqref{eq2}.\\ 
        Get inference result from $AC$.\\ 
        Continue.\\ \label{line12}
    }
    Get current bandwidth reduction ratio $\Delta B$.\\  \label{line13}
    Estimate adjusted quantization $Q^*$ according to Eq. \eqref{eq4}.\\ 
    Quantize $T^f$ with $Q^*$ and send to cloud.\\  \label{line14}
}
\end{algorithm}

COACH incorporates an innovative layer-wise offline model partitioning with quantization component, designed to optimally distribute computational resources for achieveing near bubble-free pipeline execution.
The offline component addresses the relatively underexplored complexity of achieving a balance between model partitioning and transmission quantization. 
We develop a recursive divide-and-conquer algorithm tailored for optimizing model partitioning and determining the appropriate quantization precision, as presented in Algorithm \ref{alg:alg1}.

To elevate transmission efficiency, COACH incorporates the Uniform Affine Quantization (UAQ) \cite{krishnamoorthi2018quantizing} technique to compress the intermediate data.
Specifically, UAQ effectively converts float32 variables to $B$-bit depth quantized data within a range of $(0, 2^B-1)$. 
This quantization allows for the efficient intermediate data transmission, which is then dequantized by the cloud server to continue the inference process. 
The selection of the optimal quantization precision is based on a dichotomous search, predicated on the understanding that a higher quantization precision correlates with improved inference accuracy. 
%
The DNN model can be formally represented as $G = (\mathbf{V}, \mathbf{E})$, where $\mathbf{V}$ represents the layers, and $\mathbf{E}$ comprises the inference data flows.
To navigate the complexity of DAG partitioning, COACH introduces the concept of cut-vertices $V_p\in\mathbf{V}$ to represent distinct partitioning strategies. 
We utilize two functions, $f(V_p)$ for computational cost and $g(V_p)$ for transmission cost, to evaluate the efficiency of partitioning strategy $V_p$ and analyze the bubbles in pipeline scheduling.
% Given the higher processing power in cloud servers, computational cost $f(V_p)$ inherently increases with more layers processed on the end device. 
The objective of the offline component in COACH is to identify an optimal partitioning with quantization strategy $V^*$, that minimizes the aggregate cost $f(V_p) + g(V_p)$, thereby maximizing the throughput and overall efficiency of pipeline execution.


Traditional collaborative inference approaches often simplify DNN models to generic DAGs, overlooking the unique characteristics of data flows and the opportunities of optimization. 
The principal challenge arises from the impracticality of exploring all possible partitions of a DAG, due to the exponential increase in the number of potential partitioning strategies as the model complexity grows.
To address the complexities of partitioning DAG topology models, we introduce a novel recursive divide-and-conquer algorithm. 
For chain topology, $V_p$ comprises a single vertex, whereas for DAG topology, $V_p$ encompasses multiple vertices.
Our algorithm transforms the complex multiple vertices partitions into a series of manageable single-vertex partitions.
As illustrated in Figure \ref{fig:partition}, the partitioning strategy is achieved by conceptually clustering parallel layers into virtual blocks, thereby shifting the focus of optimization towards a more manageable chain topology. 
% This approach leverages recursive divide-and-conquer to efficiently identify optimal partitioning with quantization strategies, enhancing system throughput in pipeline execution while minimizing the latency of pipeline collaborative inference.


In Algorithm \ref{alg:alg1}, the offline component starts with evaluating the computational and transmission costs of each layer in the DNN model $G$, essential for calculating computation and transmission cost functions $f$ and $g$ (Line \ref{line1}).
To simplify the exploration of optimal strategy, the algorithm divides the complex DAG topology into more manageable chain topology segments, initiating a search space $F$ for recursive analysis. 
COACH then clusters parallel layers into virtual blocks for model $G$, forming a chain flow $B_g$, which is added to the search space as $F = \{B_g\}$ (Line \ref{line2}).
Subsequently, our algorithm proceeds by iteratively evaluating each chain flow $B$ within search space $F$ to identify the corresponding optimal partitioning with quantization strategy $V_B$.
Within the context of each chain flow $B$, the algorithm employs a dichotomous search to determine the appropriate quantization precision for each block $b$.
This allows for the calculation of both the computational cost $f(V_B)$ and transmission costs $g(V_B)$, after which $V_B$ is refined based on pipeline performance (Lines \ref{line4}-\ref{line5}). 
Virtual blocks within each chain flow $B$ are then recursively integrated into the search space $F$, optimizing the model as a manageable chain topology.
After completing the exploration of $B$, the optimal strategy $V^*$ is updated with $V_B$ (Lines \ref{line6}-\ref{line7}). 
Finally, upon fully exploring the search space $F$, the algorithm determines the most effective partitioning with quantization strategy $V^*$. 
For a DAG model comprising $n$ parallel data flows, each with $c$ independent layers, the conventional approach exhibits a time complexity of $O(c^n)$. In contrast, our algorithm achieves a significantly reduced time complexity of $O(cn)$.

\begin{figure}[t]
\centering
\includegraphics[width=0.4\textwidth]{chap3/pic/partition.pdf}
\vspace{-1mm}
\caption{Illustrating DNN partitioning with virtual blocks.} 
\label{fig:partition}\vspace{-4mm}
\end{figure}

Figure \ref{fig:partition} provides a visual representation of our algorithm in simplifying the partitioning challenge.
The DAG, consisting of layers $\mathbf{V} = \{v_1, v_2, \ldots, v_9\}$, features virtual blocks $B_1$ and $B_2$, where $B_1 = \{v_2, v_3, \ldots, v_8\}$ and $B_2 = \{v_5, v_6, v_7, v_8\}$.
This restructuring transforms the DAG into a streamlined chain topology of $\{v_1, {B_1}, v_9\}$, thereby facilitating the optimization process to determine the optimal partitioning with quantization strategy $V^0_0$.
Within the virtual block $B_1\neq \emptyset$, we delineate two principal data flows for further analysis.
The data flow $\{v_2, v_3, v_4, v_8\}$ represents a straightforward partitioning scenario, suitable for implementing the strategy $V^1_0$. 
Conversely, the data flow $\{v_2, v_5, v_6, v_7, v_8\}$ necessitates cluster into $\{v_5, B_2\}$ and aligns with the strategy $V^1_1$. 
Subsequent refinement leads to the determination of optimal strategies $V^2_0$ and $V^2_1$ for the parallel data flows after exploring $B_2$. 
The comprehensive search across $[V^0_0,\{V^1_0, V^1_1\}, \{V^1_0, V^2_0, V^2_1\}]$ yields the ultimate optimal partitioning and quantization strategy $V^*$.
This strategy affords a polynomial time solution for identifying optimal partitions within complex data flows, significantly bolstering the inference process.


==> chap3/1/alg2.tex <==
% \vspace{-3mm}
\subsection{Online Inference Scheduling Component}
\label{subs:alg2}

In collaborative inference, especially within mobile computing, the challenge of dynamic network conditions has a significant influence on intermediate data transmission.
Recognizing the correlations in intermediate data, where new data often closely resembles previously transmitted data, we introduce an online inference scheduling component with
a context-aware acceleration strategy. 
The key is to implement an approximate cache \cite{li2021boosting}, designed to exploit these data correlations for real-time optimization of inference latency and throughput in dynamic environments, presented as the online acceleration component in Algorithm \ref{alg:alg1}.
  
\textbf{Approximate Cache Mechanism.} 
The online inference scheduling component incorporates a cache mechanism that intelligently adapts to fluctuating network conditions and system loads.
By employing an early-exit policy with cache, COACH exploits the temporal locality and enables the reuse of computational results.
Moreover, the quantization adjustment leverages the spatial locality of inference tasks.
To manage large volumes of intermediate data efficiently, COACH employs the Global Average Pooling (GAP) function \cite{lin2013network}. 
GAP processes intermediate data to generate \textit{task features}, which are concise feature vectors encapsulating the essential characteristics. 
Applied to intermediate data with dimensions $\left< C \times H \times W \right>$, the GAP function results in a task feature with reduced dimension $\left< C \right>$, where $C$ represents the number of channels, $H$ and $W$ are the spatial dimensions.
This dimensional reduction focuses on the core characteristics of the data, thereby enhancing the efficiency of the storage and retrieval processes within the approximate cache. 
To further facilitate the process of making similarity-based decisions, the approximate cache maintains a \textit{task feature center} for each label.
These task feature centers are initially warmed up and dynamically updated with task features, optimizing the effectiveness in supporting efficient and accurate inference processes of approximate cache.


\textbf{Task Similarity and Separability.} 
The ability to precisely evaluate data correlations including temporal locality and spatial locality between current and preceding tasks is critically important.
For assessing similarity, we employ the cosine distance metric \cite{nguyen2010cosine} for comparing task features with the task feature centers within the approximate cache, establishing similarity degrees $\mathbf{T} = \{t_j\}, j\in\{0,\ldots,n\}$ for each label.
The similarity degree for label $j$ is formalized as:
\begin{equation}
    t_j = \xi(F, T^c_j) \in [0,1],
\end{equation}    
where function $\xi(\cdot)$ represents the cosine similarity function \cite{nguyen2010cosine}. 
Let $t_j$ indicate the similarity degree, where $t_j=1$ signifies perfect similarity and $t_j=0$ indicates no similarity.
The approximate cache remains a true reflection of the ongoing conditions by gradually integrating new task features, thereby mitigating the potential impact of data biases.
The approximate cache is updated for label $j$ as follows:
\begin{equation}\label{eq2}
    T^c_j = \frac{m_jT^c_j+T^f_j}{m_j+1} \in [0,1],
\end{equation}
where $m_j$ denotes the count of tasks, $T^c_j$ is the task feature center, and $T^f_j$ is the current task feature associated with label $j$.
Moreover, to effectively harness both time and spatial localities for enhancing early-exit policies and quantization adjustments, we introduce the concept of task separability $S$ as:
\begin{equation}
    S = (t_H-t_{SH})\cdot \frac{t_H}{t_{SH}},
\end{equation}   
where $t_H$ and $t_{SH}$ are the highest and second highest degrees within similarity degrees $\mathbf{T}$, respectively.
A higher task separability $S$ indicates a strong pronounced data correlation, which plays a crucial role in context-aware acceleration.


\textbf{Context-Aware Acceleration.} 
Our context-aware acceleration strategy incorporates an early-exit policy, which leverages task separability $S$ to evaluate whether the conditions are satisfied for early termination in the collaborative inference process (Lines \ref{line11}-\ref{line12} in Alg. \ref{alg:alg1}).
Specifically, a caching threshold $S_{ext}$ is predefined with the calibration dataset $D$ to maintain an accuracy loss threshold of 0.5\%, ensuring the QoS in early-exit policy \cite{almeida2022dyno}.
When the task separability $S$ surpasses the cache threshold $S_{ext}$, it indicates that the collaborative inference process meets the criteria for early conclusion.
The decision-making process for early-exit policy is formalized as follows:
\begin{equation}
    \text{result} = \underset{j \in \{0, \ldots, n\}}{\arg\max}\{t_j\in\mathbf{T}\},
\end{equation}   
where the result is determined by identifying the maximum similarity degree among all labels within $\mathbf{T}$.
The early-exit policy ensures decisions are made based on the most relevant and similar data features, optimizing efficiency while maintaining accuracy standards.


In addition, the context-aware acceleration strategy also incorporates quantization adjustment, leveraging similarity degrees $\mathbf{T}$, task separability $S$ and real-time bandwidth reduction ratio $\Delta B$ (Lines \ref{line13}-\ref{line14}).
The quantization adjustment is founded on the understanding that higher similarity degree and separability permit a more aggressive quantization strategy without compromising the integrity of the data.
The quantization step for each label, denoted as ${\Delta Q} = \{\Delta Q_0, \Delta Q_1, \ldots, \Delta Q_n\}$, is initially determined with calibration dataset as an adjustment baseline.
The closer a task feature is to the task center, the more aggressive the adjustment with the quantization step can be to minimize transmission costs.
The adjusted quantization precision for task transmission, denoted as $Q^*$, is illustrated by the formula:
\begin{equation}\label{eq4}
    Q^* = \lceil V^* - \Delta B e^{-S\|\mathbf{T}\|_2}\Delta Q_{\max} \rceil,
\end{equation}
where $V^*$ represents the base quantization precision in the offline partitioning with quantization strategy, $\Delta Q_{\max}$ specifies the maximum quantization step allowable for the current task feature in $\Delta Q$, and $\Delta B$ is the current bandwidth reduction ratio in comparison to the initial bandwidth. 
This formula facilitates aggressive, yet data-preserving, quantization adjustments, tailored to the specific context and network conditions in the inference stage.
% By further minimizing pipeline bubbles, the quantization adjustment is pivotal in enhancing the efficiency of pipeline scheduling in dynamic network conditions.

==> chap3/1/overview.tex <==
\subsection{System Overview}

To enhance the effectiveness of collaborative inference, we focus on refining the collaborative process and leveraging data correlations. %bubble-free pipeline execution
We introduce COACH, a near bubble-free collaborative inference framework to handle the complexities of DNN models and dynamic network, ensuring efficient resource utilization while maintaining accuracy. 
The inference process is segmented into three stages: initial model processing on the end device, intermediate data transmission to the cloud, and final model computation on the cloud \cite{kang2017neurosurgeon}. 
Utilizing a multi-threaded approach, COACH concurrently manages computation and transmission, preserving a fluid pipeline flow and minimizing bubbles in pipeline scheduling.

The pipeline scheduling in COACH prevents bottlenecks by allowing computational and communication stages to occur concurrently and independently, achieveing near bubble-free pipeline scheduling through overlapping tasks effectively. 
%
The relationship between model partitioning strategy and quantization precision exhibits a reciprocal influence, as different layers require specific quantization precisions \cite{almeida2022dyno}.
COACH introduces an \textit{offline model partitioning with quantization component}, aimed at identifying the proper model partitioning and quantization strategy to ensure minimizing pipeline bubbles and reduce inference latency.
The \textit{online adaptive scheduling component} in COACH identifies data correlations and employs a special caching mechanism to explore the optimizing opportunities in pipeline execution.
This online component enables early-exit policy and quantization adjustment, thereby dynamically stabilizing the pipeline execution with network fluctuations.

\begin{figure}
    \centering
    \includegraphics[width=0.45\textwidth]{chap3/pic/overview.pdf}
    \vspace{-2mm}
    \caption{Overview and workflow of COACH.} 
    \label{fig:workflow}
    \vspace{-5mm}
\end{figure}

As illustrated in Fig.~\ref{fig:workflow}, COACH starts with the offline model partitioning with quantization component (\circled{1}), acquiring system profiles and a calibration dataset.  
The offline component involves devising an efficient partitioning strategy and assessing various quantization precisions to fine-tune pipeline scheduling, ensuring computational resources are utilized to their fullest potential.
After that, the DNN model is deployed on both the end device and cloud server, setting the stage for the collaborative inference execution with minimizing bubbles pipeline scheduling
%
During the inference process, input tasks are initially processed through the partitioned model on the end device(\circled{2}), generating intermediate data. 
Subsequently, the online adaptive scheduling component (\circled{3}) leverages a cache mechanism to evaluate the potential status of the intermediate data, which implements an early-exit policy and quantization adjustment.
Once the early-exit condition is met (\eg, exceeding a given cache threshold), the inference process will terminate at the end device and immediately generate the result (\circled{4}). 
%
Otherwise, COACH adjusts the quantization precision of the intermediate data, taking into account data correlations and bubbles in pipeline execution (\circled{5}).
The cloud server performs dequantization and completes the remaining computations and returns the inference results to the end device (\circled{6}), thereby completing the collaborative inference process.

